On the positivity of twisted $L^2$-torsion for 3-manifolds

For any compact orientable irreducible 3-manifold $N$ with empty or incompressible toral boundary, the twisted $L^2$-torsion is a non-negative function defined on the representation variety $\operatorname{Hom}(\pi_1(N),\operatorname{SL}(n,\mathbb C))$. The paper shows that if $N$ has infinite fundamental group, then the $L^2$-torsion function is strictly positive. Moreover, this torsion function is continuous when restricted to the subvariety of upper triangular representations.

==> trash.tex <==
\begin{pf}
To prove convexity, we only need to verify convexity for arbitrary two variables. Namely, it suffices to prove the following inequality
\[\left(V_{\phi_1,\phi_2}(r_1,s_1)\right)^\theta\cdot\left(V_{\phi_1,\phi_2}(r_2,s_2)\right)^{1-\theta}\geqslant V_{\phi_1,\phi_2}(r_1^\theta r_2^{1-\theta},s_1^\theta s_2^{1-\theta})\]
for all $\phi_1,\phi_2\in H^1(G;\R)$ and $r_1,r_2,s_1,s_2>0$, $\theta\in(0,1)$.

We assume that $r_1\not=r_2$ since that case has been proved by lemma \ref{single-variable}. Again by proposition \ref{single-variable}, for any real number $\lambda$ we have
\[\left(V_{\phi_1+\lambda\phi_2,\phi_2}(r_1,s)\right)^\theta\cdot\left(V_{\phi_1+\lambda\phi_2,\phi_2}(r_2,s)\right)^{1-\theta}\geqslant V_{\phi_1+\lambda\phi_2,\phi_2}(r_1^\theta r_2^{1-\theta},s).\]
We also know the identity
\[V_{\phi_1+\lambda\phi_2,\phi_2}(r,s)=V_{\phi_1,\phi_2}(r,r^\lambda s),\]
so we get an inequality
\[\left(V_{\phi_1,\phi_2}(r_1,r_1^\lambda s)\right)^\theta\cdot\left(V_{\phi_1,\phi_2}(r_2,r_2^\lambda s)\right)^{1-\theta}\geqslant V_{\phi_1,\phi_2}(r_1^\theta r_2^{1-\theta},(r_1^\lambda s)^\theta\cdot(r_2^\lambda s)^{1-\theta}).\]
Since $r_1\not=r_2$, given any two positive real numbers $s_1,s_2$ we can solve the equation
\[r_1^\lambda s=s_1,\quad r_2^\lambda s=s_2.\]
This proves the claim.
\end{pf}


We are going to focus on two pair of variables $(\phi_i,\phi_j),\ (t_i,t_j)$ and freeze other variables. Namely, We consider $V_{\phi_i,\phi_j}(t_i,t_j):=V_\Phi(T)$ as a map with variables $(\phi_1,\phi_2,t_1,t_2)\in H^1(G;\R)\times H^1(G;\R)\times \R_+\times \R_+$.

\begin{lem}\label{single-variable}
For any $\theta\in(0,1)$, we have the inequality
\[\left(V_{\phi_1,\phi_2}(r_1,s)\right)^\theta\cdot\left(V_{\phi_1,\phi_2}(r_2,s)\right)^{1-\theta}\geqslant V_{\phi_1,\phi_2}(r_1^\theta r_2^{1-\theta},s)\]
holds for all $\phi_1,\phi_2\in H^1(G;\R)$ and $r_1,r_2,s>0$.
\end{lem}
\begin{pf}
The inequality follows from the convexity part of proposition \ref{coordinate-convex}.
\end{pf}


Let's first decompose $N$ into smaller pieces via JSJ-decomposition, with the help of the sum formula. It is known that any JSJ component of $N$ is either hyperbolic or a Seifert-fibering space.

\begin{thm}
Let $N_1,\cdots,N_r$ be the JSJ components in any JSJ decomposition of $N$. For any $i=1,\cdots,r$, denote by $\rho_i=\rho|_{\pi_1(N_i)}$ the restriction of $\rho$, then we have
\[\tautwo(N,\rho)=\prod_{i=1}^n\tautwo(N_i,\rho_i).\]
\end{thm}

\begin{pf}
It is a immediate consequence of \cref{TorusTorsionFormula} and \cref{BasicProppertyTorsion}.
\end{pf}
 The fundamental group of $M$ has the presentation:
\[\pi_1(M)=\langle a_1,b_1,\cdots,a_g,b_g,e_1,\cdots,e_b,f_1,\cdots,f_{k-1},h:hx=xh,\forall x\in\pi_1(M),\  f_i^{p_i}h^{q_i}=1\rangle.\]
